Tracemax: A Novel Single Packet IP Traceback Strategy for Data-Flow Analysis

The identification of the exact path that packets are routed on in the network is quite a challenge. This paper presents a novel, efficient traceback strategy named Tracemax in context of a defense system against distributed denial of service (DDoS) attacks. A single packet can be directly traced over many more hops than the current existing techniques allow. In combination with a defense system it differentiates between multiple connections. It aims to letting non-malicious connections pass while bad ones get thwarted. The novel concept allows detailed analyses of the traffic and the transmission path through the network. The strategy can effectively reduce the effect of common bandwidth and resource consumption attacks, foster early warning and prevention as well as higher the availability of the network services for the wanted customers.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> content/problem.tex <==
\section{PROBLEM DESCRIPTION}


==> content/szenarioold.tex <==
\section{SCENARIO}\label{scenario}
%As we know from other defence strategies against DDoS, the problem can not be solved at the end user, the victim.
%The novel defence and traceback strategy can be separated in steps, where every step improves the strength. 
We imagine on a scenario that someone starts attacking a user at a different ISP zone than himself.
If the victim is under pressure of a network consumption attack, the massive inbound traffic blocks a normal communication to other systems, which could support to defend. Such attacks can be very easily detected at the end user or vicitim \cite{Li2003, Sanmorino13}. At this moment, the host system of the victim has still enough resources to analyze the incoming traffic and to filter wrong and normal requests. Otherwise, the victim has to send these data to an Host Intrusion Detection System or a Network Intrusion Detection System, which would detect by its own that the server is under attack. Depending on the signature of the bad request, which could be something very simple like IP addresses, Ports or special Protocols, the system will store this information with a time stamp in a database. The victim or the operator of the local network activate the traceback configuration to find the source of the attack and start defending against it. The router propagate the activation through the entire network by themself, also to the ISP routers. Therefore, an cooperation with the ISP is necessary. ISPs should be self interested in reducing their load on their network and defending against bandwidth consumption attacks. These configuration messages are cryptographic authenticated. Furthermore, the signature of the bad packets is also propagated. The routers use this signature to start filtering and blocking such incoming messages. After the configuration of the router, all messages will be traced. The traceback information is prepared in a kind that the victim, ISP and network management is able to address the forensic needs of law enforcement. Figure \ref{TracebackAttacker} shows an example of necessary components for traceback and the different attack paths of the attacker.


%After that, in the first step, this information is send to the local router or firewall to start blocking these requests. This is still possible, because the victim is able to send packets, but not to receive. Maybe an intelligent router would manage the queue to priorize the answer information of it self than the outside incoming packets to communicate with the victim.
%The victim configure with the outgoing messages the local routers and firewalls. But this has to be secured by the Communication Protocol that the victim is only allowed to configure the rules set for the own incoming and outgoing packets. Especially, it’s only allowed to create an additional rule set than the from the network administrator defined one. There have to be a trusted communication that no other in the local network is possible to do it form it, otherwise an other DoS would be possible.

\vspace{1mm}
 \begin{figure}[htb]
 {
 \centering
 \includegraphics[width=0.5\textwidth]{fig/SzenarioP.png}
 \caption{Traceback of an attacker.}
\label{TracebackAttacker}
 }
 \end{figure}

